Efficient Symmetry Reduction and the Use of State Symmetries for Symbolic Model Checking

One technique to reduce the state-space explosion problem in temporal logic model checking is symmetry reduction. The combination of symmetry reduction and symbolic model checking by using BDDs suffered a long time from the prohibitively large BDD for the orbit relation. Dynamic symmetry reduction calculates representatives of equivalence classes of states dynamically and thus avoids the construction of the orbit relation. In this paper, we present a new efficient model checking algorithm based on dynamic symmetry reduction. Our experiments show that the algorithm is very fast and allows the verification of larger systems. We additionally implemented the use of state symmetries for symbolic symmetry reduction. To our knowledge we are the first who investigated state symmetries in combination with BDD based symbolic model checking.

==> eptcsdata.tex <==
\providecommand{\event}{Angelo Montanari, Margherita Napoli, Mimmo Parente (Eds.)\\ Proceedings of GandALF 2010}
\providecommand{\volume}{25}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{173}
\providecommand{\eid}{17}

